The finite cohesiveness principle

We investigate the logical strength of the cohesiveness principle when restricted to finite sequences of sets, denoted by fin-COH, over different base theories. Our main result shows that fin-COH entails $I\Sigma_1^0$ over the weaker base theory $RCA_0^*$, thereby answering a question posed by Fiori-Carones, Ko{\l}odziejczyk and Kowalik. In addition, we show that fin-COH is not provable over $WKL_0$.

==> macros.tex <==
% macros.tex
\makeatletter
\usepackage{todonotes}
% \usepackage[disable]{todonotes}
\usepackage{enumitem}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{cite}
\usepackage{xcolor}
\usepackage[hidelinks]{hyperref}
% \hypersetup{
%  colorlinks,
%  linkcolor={red!40!black},
%  citecolor={blue!40!black},
%  urlcolor={blue!40!black}
% }


\theoremstyle{definition}
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{qn}[thm]{Question}
\newtheorem{prob}[thm]{Problem}
\newtheorem{question}[thm]{Question}
\newtheorem{definition}[thm]{Definition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem*{observation}{Observation}
\newtheorem{notation}[thm]{Notation}
\newtheorem{problem}[thm]{Problem}
\newcommand{\cod}[2]{\mathnoun{Cod}({#1}/{#2})}
\newcommand{\wrd}{\mathnoun{WR}}
\newcommand{\clref}[1]{(\ref{#1})}
\renewcommand{\rm}[1]{\mathrm{#1}}
\renewcommand{\bf}[1]{\textbf{#1}}

% \let\clref\eqref
\newcommand{\tfaeenum}
 {\renewcommand{\theenumi}{\roman{enumi}}%
  \renewcommand{\labelenumi}{(\theenumi)}}
\theoremstyle{remark}
\newtheorem{rmk}[thm]{Remark}
\newtheorem*{remark}{Remark}
\newtheorem*{claim}{Claim}
\newtheorem*{proofofclaim}{Proof of Claim}

\renewcommand{\today}{\number\day~%
 \ifcase \month \or January\or February\or March\or April\or May\or June\or
   July\or August\or September\or October\or November\or December\fi,
 \number\year}
% \newcommand{\mar}[1]{\marginpar{\raggedright\mbox{}#1}}
\newcommand{\mar}[1]{\ifdraft\marginpar{\raggedright\mbox{}#1}\fi}
\newif\ifdraft
\let\phi\varphi
\let\leq\leqslant
\let\geq\geqslant
\let\mathnoun\mathrm
\let\defm\emph
% \let\clref\eqref
\let\then\rightarrow
\let\Then\Rightarrow
\let\nsc\leftrightarrow
\let\Nsc\Leftrightarrow

\newcommand{\qThen}{\quad\Then\quad}
\newcommand{\qNsc}{\quad\Nsc\quad}
\newcommand{\qand}{\quad\text{and}\quad}
\newcommand{\hyp}{\text{-}}
\newcommand{\excf}[1]{\exists^{\cf}{#1}\ }


\newcommand{\fa}[1]{\forall{#1}\ }
\newcommand{\Q}[1]{\mathnoun{Q}{#1}\ }
\newcommand{\Qklt}[3]{Q_{#1}{#2}<{#3}\ }
\newcommand{\Qbar}[1]{\ov{\mathnoun{Q}}{#1}\ }
\newcommand{\ex}[1]{\exists{#1}\ }
\newcommand{\exi}[1]{\ex{!{#1}}}
\newcommand{\falt}[2]{\fa{{#1}<{#2}}}
\newcommand{\exlt}[2]{\ex{{#1}<{#2}}}
\newcommand{\fale}[2]{\fa{{#1}\leq{#2}}}
\newcommand{\exle}[2]{\ex{{#1}\leq{#2}}}

\newcommand{\exlg}[2]{\ex{{#1}>{#2}}}
\newcommand{\falg}[2]{\fa{{#1}>{#2}}}

\newcommand{\restdto}[1]{\mathclose{\restriction_{#1}}}
\newcommand{\elemsub}{\preccurlyeq}
\newcommand{\elemext}{\succcurlyeq}
\newcommand{\elemsubneq}{\precneqq}
\newcommand{\elemextneq}{\succneqq}
\newcommand{\powset}{\mathscr{P}}
\newcommand{\setm}{\setminus}
\newcommand{\restd}{\mathclose{\upharpoonright}}
\newcommand{\ov}{\overline}
\newcommand{\fain}[2]{\fa{{#1}\in{#2}}}
\newcommand{\exin}[2]{\ex{{#1}\in{#2}}}

\newcommand{\IN}{\mathbb{N}}
\newcommand{\co}{\mathnoun{co}\hyp}
\newcommand{\NP}{\mathnoun{NP}}
\newcommand{\proves}{\mathrel{\mathrel|\joinrel\mathrel-}}

\let\sup\undefined
\DeclareMathOperator{\sup}{sup}
% \newcommand{\restdto}[1]{\mathclose{\restriction_{#1}}}
\newcommand{\rt}{\mathnoun{RT}}
\newcommand{\rd}{\mathnoun{R}}
\newcommand{\php}{\mathnoun{PHP}}
\newcommand{\cf}{\mathnoun{cf}}
\newcommand{\ee}{\mathnoun{e}}
\newcommand{\rr}{\mathnoun{r}}
\newcommand{\lang}{\mathcal L}
\newcommand{\Lone}{\lang_1}
\newcommand{\Ltwo}{\lang_2}
\renewcommand{\exp}{\mathnoun{exp}}
\newcommand{\ind}{\mathnoun{I}}
\newcommand{\bd}{\mathnoun{B}}
\newcommand{\pfn}{\mathnoun{P}}
\newcommand{\PA}{\mathnoun{PA}}
\newcommand{\defset}{\mathnoun{Def}}
\newcommand{\PAminus}{\PA^{-}}
\newcommand{\WKL}{\mathnoun{WKL}}
\newcommand{\ADS}{\mathnoun{ADS}}
\newcommand{\RT}{\mathnoun{RT}}
\newcommand{\SRT}{\mathnoun{SRT}}
\newcommand{\CRT}{\mathnoun{CRT}}

\newcommand{\ACA}{\mathnoun{ACA}}
\newcommand{\RCA}{\mathnoun{RCA}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\finsep}{\mathnoun{fin}\hyp\Sigma_2^0\hyp\mathrm{Separation}}
\newcommand{\sep}{\Sigma_2^0\hyp\mathrm{Separation}}
\newcommand{\fincoh}{\mathnoun{fin}\hyp\mathnoun{COH}}
\newcommand{\coh}{\mathnoun{COH}}
\newcommand{\nmrl}[1]{\underline{#1}}
\newcommand{\Sat}{\mathnoun{Sat}}
\newcommand{\Con}{\mathnoun{Con}}
\newcommand{\tuple}[1]{\langle#1\rangle}
\newcommand{\Ack}[1]{\mathnoun{Ack}(#1)}
\newcommand{\inAck}{\in\Ack}
\newcommand{\notinAck}{\notin\Ack}
\renewcommand{\u}{\mathcal{U}}
\newcommand{\f}{\mathcal{F}}
\newcommand{\g}{\mathcal{G}}
\newcommand{\ultp}{\mathcal{F}/\mathcal{U}}
\newcommand{\Th}{\mathnoun{Th}}
% \newcommand{\dom}{\mathnoun{dom}}
% \newcommand{\range}{\mathnoun{range}}
\newcommand{\SSy}{\mathnoun{SSy}}
\newcommand{\Diagel}{\mathnoun{Diag}_{\mathnoun{el}}}
% \newcommand{\len}{\mathnoun{len}}
\DeclareMathOperator{\len}{len}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\range}{range}


\makeatother
\endinput

